The Vienna Architecture Description Language

The Vienna Architecture Description Language (VADL) is a powerful processor description language (PDL) that enables the concise specification of processor architectures. From a single VADL processor specification, the VADL compiler can automatically generate a wide range of artifacts required for rapid design space exploration. These include assemblers, compilers, linkers, functional and cycle-accurate instruction set simulators, synthesizable hardware description language (HDL) specifications, as well as test cases and documentation. A distinctive feature of VADL is the separation of the instruction set architecture (ISA) specification from the microarchitecture (MiA) specification. This decoupling gives users the flexibility to combine various ISAs with different MiAs, offering a versatile approach to processor design. In contrast to existing PDLs, VADL's MiA specification operates at a higher level of abstraction, enhancing the clarity and simplicity of the design process. Notably, using a single ISA specification, VADL streamlines compiler generation and maintenance by eliminating the need for intricate compiler-specific knowledge. Because the original VADL implementation is subject to restrictive licensing, the open-source implementation OpenVADL was initiated. This article introduces VADL, compares the original implementation with the ongoing OpenVADL development, describes the generator techniques in detail, and demonstrates both the expressiveness of the language and the performance of the generators in an empirical evaluation. The evaluation highlights the conciseness of VADL and the efficiency of the generated artifacts. Finally, the viability of OpenVADL for design space exploration is demonstrated in a case study on CRC32 checksum computation for the RISC-V ISA.

==> src-evalparser.tex <==



==> src-evalsimbuild.tex <==
\subsection{Evaluation of the Simulator Build Times}
\label{sec:evalsimbuild}

For productive experimentation and design space exploration
it is beneficial to have short simulator build times.
Depending on the task at hand, a short edit-build-run cycle also
can  influence the decision which kind of simulator to choose.

We measured the generation time of the RISC-V generators used
in our evaluation for comparison.
Table~\ref{tab:sim-build-times} shows the complete
build times of the simulators for
the RV32IM specification
as reported by \texttt{bash} in seconds.
The generation of \ac{ISS} and \ac{CAS} include the
\ac{VADL} execution time and the build time of the emitted code.
The generation of \ac{HDL} includes everything from
the \ac{VADL} execution time, the translation from Chisel to
Verilog, the execution time of Verilator, to the build time
of the code emitted by Verilator.

\begin{table}[!ht]
\centering
\caption{Build times of RISC-V RV32IM simulators}
\label{tab:sim-build-times}
\begin{tabular}{|l|r|} \hline
simulator               & build time in s \\ \hline
ISS              & 6.686     \\
CAS 1 stage      & 10.779    \\
CAS 2 stages     & 14.357    \\
CAS 3 stages     & 12.480    \\
CAS 5 stages     & 12.348    \\
HDL 5 stages     & 58.599    \\ \hline
\end{tabular}
\end{table}

